From CCS to CSP: the m-among-n Synchronisation Approach

We present an alternative translation from CCS to an extension of CSP based on m-among-n synchronisation (called CSPmn). This translation is correct up to strong bisimulation. Unlike the g-star renaming approach ([4]), this translation is not limited by replication (viz., recursion with no nested parallel composition). We show that m-among-n synchronisation can be implemented in CSP based on multiway synchronisation and renaming.

==> eptcsdata.tex <==
\providecommand{\firstpage}{60}
\providecommand{\publicationstatus}{V. Castiglioni and C. A. Mezzina (Eds): Combined Workshop on \\ Expressiveness in Concurrency and Structural Operational Semantics 2022 \\ (EXPRESS/SOS 2022).\\
EPTCS 368, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.368.4}{10.4204/EPTCS.368.4}}

